Faster Offloads by Unloading them -- The RDMA Case

From hardware offloads like RDMA to software ones like eBPF, offloads are everywhere and their value is in performance. However, there is evidence that fully offloading -- even when feasible -- does not always give the expected speedups. Starting from the observation that this is due to changes the offloads make -- by moving tasks from the application/CPU closer to the network/link layer -- we argue that to further accelerate offloads, we need to make offloads reversible by unloading them -- moving back part of the offloaded tasks. Unloading comes with a set of challenges that we start answering in this paper by focusing on (offloaded) RDMA writes: which part of the write operation does it make sense to unload? how do we dynamically decide which writes to execute on the unload or offload path to improve performance? how do we maintain compatibility between the two paths? Our current prototype shows the potential of unloading by accelerating RDMA writes by up to 31%.

==> figures/plot_config.tex <==
% Define the colors
\definecolor{TabBlue}{rgb}{0.1216,0.4667,0.7059}  % Blue
\definecolor{TabOrange}{rgb}{1.0000,0.4980,0.0549}  % Orange
\definecolor{TabGreen}{rgb}{0.1725,0.6275,0.1725}  % Green
\definecolor{TabRed}{rgb}{0.8392,0.1529,0.1569}  % Red
\definecolor{TabPurple}{rgb}{0.5804,0.4039,0.7412}  % Purple
\definecolor{TabBrown}{rgb}{0.5490,0.3373,0.2941}  % Brown
\definecolor{TabPink}{rgb}{0.8902,0.4667,0.7608}  % Pink
\definecolor{TabGray}{rgb}{0.4980,0.4980,0.4980}  % Gray
\definecolor{TabYellow}{rgb}{0.7373,0.7412,0.1333}  % Yellow
\definecolor{TabCyan}{rgb}{0.0902,0.7451,0.8039}  % Cyan

% Use the defined colors in the colormap
\pgfplotsset{
  colormap={Tab10}{
    color=(TabOrange)
    color=(TabGreen)
    color=(TabBlue)
    color=(TabRed)
    color=(TabPurple)
    color=(TabBrown)
    color=(TabPink)
    color=(TabGray)
    color=(TabYellow)
    color=(TabCyan)
  }
}

\pgfplotsset{
    legend style={draw=none, fill=white, fill opacity=0, draw opacity=1, text opacity=1}, % remove legend border
    legend cell align={left}, %left align legent entries
    legend pos=north west, % legend inside, bottom right
    axis x line*=bottom, % no top axis
    axis y line*=left, % no right axis
    colormap name=Tab10, % use colors from the top of the file
    cycle list={[of colormap]}, % addplot+ to default on colormap
    bar cycle list/.style={cycle  list={%
        {TabOrange, fill=TabOrange!75!white},
        {TabGreen, fill=TabGreen!75!white},
        {TabBlue, fill=TabBlue!75!white},
        {TabRed, fill=TabRed!75!white},
        {TabPurple, fill=TabPurple!75!white},
        {TabBrown, fill=TabBrown!75!white},
        {TabPink, fill=TabPink!75!white},
        {TabGray, fill=TabGray!75!white},
        {TabYellow, fill=TabYellow!75!white},
        {TabCyan, fill=TabCyan!75!white},%
      }
    },
    ymin=0.0,
    ymax=6,
    % enlarge x limits=0.5,
    % enlarge x limits = true,
    % enlarge x limits=1,
    % xmin=0,
    legend style={draw=none, font=\small, fill=white, fill opacity=0, draw opacity=1, text opacity=1}, % remove legend border
    height=\linewidth/2,
    width=\linewidth,
    table/col sep=comma,
    label style={font=\normalsize},
    legend image code/.code={
        \draw[mark repeat=2,mark phase=2]
            plot coordinates {
                (0cm,0cm)
                (0.15cm,0cm)        %% default is (0.3cm,0cm)
                (0.3cm,0cm)         %% default is (0.6cm,0cm)
            };%
    },
    % legend style={at={(0.55, 0.65)},anchor=north west},
    legend style={
        at={(0.5,1.0)},
        anchor=center,
        legend columns=-1,
        /tikz/every even column/.append style={column sep=0.5em}
    },
    every axis plot/.append style={thick}, % thick lines,
    every lineplot plot/.append style={xmin = 0},
    scaled y ticks = false,
    scaled x ticks = false,
    ybar style/.style={ % ybar specific options
       enlarge x limits={abs=0.5} % +half a group on each direction to avoid cutting off groups
    },
    % Automatically apply the style to ybar plots
    /pgfplots/ybar/.append style=ybar style % avoid cutting off first set of bars
}

\pgfplotsset{
    filter discard warning=false,
    discard if not/.style 2 args={
        x filter/.append code={
            \edef\tempa{\thisrow{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}

\makeatletter
\pgfplotstableset{
    discard if not/.style 2 args={
        row predicate/.append code={
            \def\pgfplotstable@loc@TMPd{\pgfplotstablegetelem{##1}{#1}\of}
            \expandafter\pgfplotstable@loc@TMPd\pgfplotstablename
            \edef\tempa{\pgfplotsretval}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \pgfplotstableuserowfalse
            \fi
        }
    }
}
\makeatother

\pgfplotsset{
    label/.initial=,
    every axis plot post/.code={%
        \pgfkeysgetvalue{/pgfplots/label}\tempValue
        \ifx\tempValue\empty
            \pgfkeysalso{/pgfplots/forget plot}%
        \else
            \expandafter\addlegendentry\expandafter{\tempValue}%
        \fi
    },
}

